Concept-RuleNet: Grounded Multi-Agent Neurosymbolic Reasoning in Vision Language Models

Modern vision-language models (VLMs) deliver impressive predictive accuracy yet offer little insight into 'why' a decision is reached, frequently hallucinating facts, particularly when encountering out-of-distribution data. Neurosymbolic frameworks address this by pairing black-box perception with interpretable symbolic reasoning, but current methods extract their symbols solely from task labels, leaving them weakly grounded in the underlying visual data. In this paper, we introduce a multi-agent system - Concept-RuleNet that reinstates visual grounding while retaining transparent reasoning. Specifically, a multimodal concept generator first mines discriminative visual concepts directly from a representative subset of training images. Next, these visual concepts are utilized to condition symbol discovery, anchoring the generations in real image statistics and mitigating label bias. Subsequently, symbols are composed into executable first-order rules by a large language model reasoner agent - yielding interpretable neurosymbolic rules. Finally, during inference, a vision verifier agent quantifies the degree of presence of each symbol and triggers rule execution in tandem with outputs of black-box neural models, predictions with explicit reasoning pathways. Experiments on five benchmarks, including two challenging medical-imaging tasks and three underrepresented natural-image datasets, show that our system augments state-of-the-art neurosymbolic baselines by an average of 5% while also reducing the occurrence of hallucinated symbols in rules by up to 50%.

==> junk.tex <==
<!-- 4. Our setting is interpretable, low-label LVLM reasoning - we extract image-grounded concepts and compose symbolic rules that are verifiable at inference properties that a fine-tuned CNN does not provide. Crucially, we operate in a very-low-data regime: rules are induced from only 50 images per class family (Tab-5), whereas the cited CNN figures assume *thousands of images*. Under the same 50-image budget, a ResNet-50 reaches 19.5 (Blood) and 22.36 (Derma), confirming DNNs need far more supervision to be competitive here. By contrast, Concept-RuleNet consistently improves over System-1 and Symbol-LLM across datasets (Tab-1) and also with a medical verifier (Tab-2), while yielding checkable rule traces and reducing hallucinated symbols. We will report these 50-image ResNet result rows (clearly marked non-interpretable) to contextualize that under equal data, CRN is both more accurate and explainable. -->


